Compressing Neural Networks: Towards Determining the Optimal Layer-wise Decomposition

We present a novel global compression framework for deep neural networks that automatically analyzes each layer to identify the optimal per-layer compression ratio, while simultaneously achieving the desired overall compression. Our algorithm hinges on the idea of compressing each convolutional (or fully-connected) layer by slicing its channels into multiple groups and decomposing each group via low-rank decomposition. At the core of our algorithm is the derivation of layer-wise error bounds from the Eckart Young Mirsky theorem. We then leverage these bounds to frame the compression problem as an optimization problem where we wish to minimize the maximum compression error across layers and propose an efficient algorithm towards a solution. Our experiments indicate that our method outperforms existing low-rank compression approaches across a wide range of networks and data sets. We believe that our results open up new avenues for future research into the global performance-size trade-offs of modern neural networks. Our code is available at https://github.com/lucaslie/torchprune.

==> fig/cifar_prune/cifar_prune_table.tex <==
\begin{tabular}{|c|c|c||ccc|ccc|ccc|ccc|ccc|}
\hline
\multirow{30}{*}{\rotatebox{90}{CIFAR10}}
& \multirow{2}{*}{Model}
& \multirow{2}{*}{\shortstack{Prune \\ Method}}
& \multicolumn{3}{c|}{$\delta=1.0\%$}
& \multicolumn{3}{c|}{$\delta=5.0\%$}
& \multicolumn{3}{c|}{$\delta=10.0\%$}
& \multicolumn{3}{c|}{$\delta=20.0\%$}
& \multicolumn{3}{c|}{$\delta=30.0\%$} \\
& &
& Top1 Acc. & CR-P & CR-F
& Top1 Acc. & CR-P & CR-F
& Top1 Acc. & CR-P & CR-F
& Top1 Acc. & CR-P & CR-F
& Top1 Acc. & CR-P & CR-F \\ \cline{2-18}
& \multirow{7}{*}{\shortstack{ResNet20 \\ \\ Top1: 91.39}}
& ALDS
& -0.41 & \textbf{17.47} & \textbf{9.08}
& -3.27 & \textbf{30.19} & 19.75
& -7.36 & \textbf{40.89} & 30.35
& -10.35 & \textbf{45.40} & 35.75
& -25.15 & 49.96 & 40.51 \\
& & PCA
& -0.06 & 2.94 & 1.36
& -4.92 & \textbf{30.26} & \textbf{29.00}
& -6.98 & 35.78 & \textbf{35.00}
& -14.77 & \textbf{45.73} & \textbf{44.60}
& -29.92 & \textbf{54.12} & \textbf{53.44} \\
& & SVD-Energy
& -0.96 & 2.99 & 1.95
& -0.96 & 2.99 & 1.95
& -7.33 & 10.74 & 9.96
& -19.13 & 17.83 & 16.84
& -28.06 & 30.40 & 29.39 \\
& & SVD
&   &   &  
& -3.30 & 2.49 & 2.57
& -3.30 & 2.49 & 2.57
& -13.78 & 10.09 & 9.59
& -25.65 & 23.86 & 23.32 \\
& & L-Rank
& -0.41 & 3.03 & 2.72
& -0.41 & 3.03 & 2.72
& -0.41 & 3.03 & 2.72
& -10.77 & 10.75 & 19.69
& -10.77 & 10.75 & 19.69 \\
& & FT
&   &   &  
& -1.33 & 2.71 & 2.44
& -7.68 & 11.11 & 10.48
& -7.68 & 11.11 & 10.48
& -22.51 & 18.41 & 19.14 \\
& & PFP
&   &   &  
& -1.68 & 2.92 & 1.57
& -1.68 & 2.92 & 1.57
& -13.20 & 10.70 & 6.86
& -29.03 & 17.65 & 12.18 \\
\cline{2-18}
& \multirow{7}{*}{\shortstack{VGG16 \\ \\ Top1: 92.78}}
& ALDS
& -0.86 & 57.72 & 36.33
& -3.54 & 67.03 & 44.97
& -6.33 & 69.68 & 47.57
& -15.04 & 72.14 & 50.45
& -24.40 & 74.31 & 52.64 \\
& & PCA
& -0.98 & \textbf{76.38} & \textbf{56.57}
& -1.95 & \textbf{80.00} & \textbf{64.14}
& -1.95 & \textbf{80.00} & \textbf{64.14}
& -1.95 & \textbf{80.00} & \textbf{64.14}
& -1.95 & \textbf{80.00} & 64.14 \\
& & SVD-Energy
& -0.94 & 3.00 & 6.87
& -4.11 & 35.98 & 41.25
& -5.74 & 41.09 & 46.12
& -18.25 & 57.74 & 60.97
& -28.48 & 64.21 & \textbf{66.47} \\
& & SVD
& -0.29 & 10.71 & 9.88
& -4.67 & 35.93 & 35.29
& -4.67 & 35.93 & 35.29
& -11.62 & 45.77 & 45.21
& -29.89 & 67.04 & \textbf{66.67} \\
& & L-Rank
& -0.51 & 10.74 & 14.58
& -4.50 & 50.10 & 41.46
& -8.08 & 64.22 & 50.45
& -18.79 & 76.38 & 60.15
& -25.67 & \textbf{80.01} & 64.78 \\
& & FT
& -0.35 & 2.77 & 2.95
& -2.67 & 10.74 & 10.88
& -8.90 & 17.75 & 17.78
& -19.14 & 24.41 & 24.24
& -19.14 & 24.41 & 24.24 \\
& & PFP
& -0.85 & 30.37 & 12.56
& -4.49 & 45.58 & 21.83
& -9.15 & 49.99 & 25.20
& -14.84 & 54.14 & 28.71
& -25.72 & 61.11 & 35.36 \\
\cline{2-18}
& \multirow{7}{*}{\shortstack{DenseNet22 \\ \\ Top1: 89.88}}
& ALDS
& +0.03 & 0.20 & 0.03
& -4.50 & \textbf{8.55} & \textbf{7.89}
& -4.50 & 8.55 & 7.89
& -16.07 & \textbf{16.06} & 15.57
& -21.54 & \textbf{22.56} & 21.42 \\
& & PCA
& -0.75 & \textbf{2.84} & \textbf{7.28}
& -0.75 & 2.84 & 7.28
& -6.60 & \textbf{10.43} & \textbf{25.25}
& -6.60 & 10.43 & \textbf{25.25}
& -6.60 & 10.43 & \textbf{25.25} \\
& & SVD-Energy
&   &   &  
&   &   &  
&   &   &  
& -10.31 & 3.04 & 4.94
& -10.31 & 3.04 & 4.94 \\
& & SVD
&   &   &  
&   &   &  
&   &   &  
&   &   &  
& -22.79 & 9.34 & 9.60 \\
& & L-Rank
&   &   &  
&   &   &  
&   &   &  
& -11.24 & 2.98 & 7.00
& -11.24 & 2.98 & 7.00 \\
& & FT
&   &   &  
&   &   &  
& -6.24 & 3.02 & 3.87
& -6.24 & 3.02 & 3.87
& -6.24 & 3.02 & 3.87 \\
& & PFP
& -0.67 & \textbf{2.82} & 3.90
& -0.67 & 2.82 & 3.90
& -0.67 & 2.82 & 3.90
& -10.64 & 10.99 & 14.12
& -10.64 & 10.99 & 14.12 \\
\cline{2-18}
& \multirow{7}{*}{\shortstack{WRN16-8 \\ \\ Top1: 95.21}}
& ALDS
& -0.83 & 64.19 & 51.53
& -4.15 & 74.25 & 62.77
& -9.85 & 78.26 & 67.58
& -14.22 & \textbf{79.97} & 69.77
& -14.22 & \textbf{79.97} & 69.77 \\
& & PCA
& -0.81 & \textbf{67.04} & \textbf{64.97}
& -3.94 & \textbf{79.97} & \textbf{77.77}
& -3.94 & \textbf{79.97} & \textbf{77.77}
& -3.94 & \textbf{79.97} & \textbf{77.77}
& -3.94 & \textbf{79.97} & \textbf{77.77} \\
& & SVD-Energy
& -0.87 & 41.08 & 34.33
& -1.67 & 54.09 & 48.91
& -1.67 & 54.09 & 48.91
& -18.17 & 69.70 & 66.45
& -29.90 & 78.26 & 75.85 \\
& & SVD
& -0.01 & 2.95 & 3.14
& -0.01 & 2.95 & 3.14
& -9.12 & 10.69 & 10.95
& -19.16 & 45.71 & 45.64
& -29.69 & 57.72 & 57.64 \\
& & L-Rank
& -0.99 & 41.09 & 46.98
& -3.29 & 54.09 & 62.65
& -5.87 & 57.74 & 66.17
& -19.26 & 64.22 & 72.30
& -19.26 & 64.22 & 72.30 \\
& & FT
& -0.28 & 10.88 & 11.59
& -3.49 & 24.54 & 24.89
& -9.15 & 30.57 & 30.81
& -14.87 & 35.91 & 36.11
& -21.89 & 41.17 & 41.26 \\
& & PFP
& -0.40 & 24.45 & 19.82
& -2.32 & 30.38 & 26.42
& -6.45 & 35.94 & 32.43
& -13.27 & 41.09 & 37.86
& -22.60 & 45.84 & 42.77 \\
\hline
\end{tabular}


==> fig/cifar_pruneablation/cifar_pruneablation_table.tex <==
\begin{tabular}{|c|c|c||ccc|ccc|ccc|ccc|ccc|}
\hline
\multirow{8}{*}{\rotatebox{90}{CIFAR10}}
& \multirow{2}{*}{Model}
& \multirow{2}{*}{\shortstack{Prune \\ Method}}
& \multicolumn{3}{c|}{$\delta=1.0\%$}
& \multicolumn{3}{c|}{$\delta=5.0\%$}
& \multicolumn{3}{c|}{$\delta=10.0\%$}
& \multicolumn{3}{c|}{$\delta=20.0\%$}
& \multicolumn{3}{c|}{$\delta=30.0\%$} \\
& &
& Top1 Acc. & CR-P & CR-F
& Top1 Acc. & CR-P & CR-F
& Top1 Acc. & CR-P & CR-F
& Top1 Acc. & CR-P & CR-F
& Top1 Acc. & CR-P & CR-F \\ \cline{2-18}
& \multirow{6}{*}{\shortstack{ResNet20 \\ \\ Top1: 91.39}}
& ALDS
& -0.46 & \textbf{18.53} & \textbf{9.41}
& -3.37 & \textbf{31.02} & \textbf{20.01}
& -7.64 & \textbf{41.77} & \textbf{31.49}
& -19.61 & \textbf{54.48} & \textbf{45.15}
& -19.61 & \textbf{54.48} & \textbf{45.15} \\
& & ALDS-Error3
& +0.01 & 4.06 & 1.74
& -4.05 & 18.62 & 13.07
& -4.05 & 18.62 & 13.07
& -16.63 & 31.06 & 27.31
& -22.06 & 36.42 & 32.87 \\
& & ALDS-Simple3
&   &   &  
& -4.84 & 4.69 & 3.40
& -4.84 & 4.69 & 3.40
& -15.90 & 18.77 & 18.42
& -23.39 & 25.84 & 26.44 \\
& & ALDS-Simple5
&   &   &  
& -4.84 & 4.69 & 3.40
& -4.84 & 4.69 & 3.40
& -15.90 & 18.77 & 18.42
& -23.39 & 25.84 & 26.44 \\
& & Messi3
&   &   &  
& -4.65 & 11.66 & 13.19
& -4.65 & 11.66 & 13.19
& -19.21 & 25.01 & 24.56
& -27.25 & 31.78 & 32.19 \\
& & SVD-Error
& -0.33 & 3.91 & 1.74
& -3.30 & 11.60 & 8.00
& -9.23 & 18.66 & 16.09
& -9.23 & 18.66 & 16.09
& -28.37 & 25.05 & 23.44 \\
\hline
\end{tabular}


==> fig/cifar_retrainablation/cifar_retrainablation_table.tex <==
\begin{tabular}{|c|c|c||ccc|ccc|ccc|ccc|ccc|}
\hline
\multirow{8}{*}{\rotatebox{90}{CIFAR10}}
& \multirow{2}{*}{Model}
& \multirow{2}{*}{\shortstack{Prune \\ Method}}
& \multicolumn{3}{c|}{$\delta=0.0\%$}
& \multicolumn{3}{c|}{$\delta=0.5\%$}
& \multicolumn{3}{c|}{$\delta=1.0\%$}
& \multicolumn{3}{c|}{$\delta=2.0\%$}
& \multicolumn{3}{c|}{$\delta=3.0\%$} \\
& &
& Top1 Acc. & CR-P & CR-F
& Top1 Acc. & CR-P & CR-F
& Top1 Acc. & CR-P & CR-F
& Top1 Acc. & CR-P & CR-F
& Top1 Acc. & CR-P & CR-F \\ \cline{2-18}
& \multirow{6}{*}{\shortstack{ResNet20 \\ \\ Top1: 91.39}}
& ALDS
& +0.12 & \textbf{64.31} & \textbf{56.46}
& -0.48 & \textbf{75.04} & \textbf{68.96}
& -0.70 & \textbf{79.03} & 71.14
& -1.96 & \textbf{87.67} & \textbf{83.13}
& -2.69 & \textbf{89.71} & \textbf{85.86} \\
& & ALDS-Error3
& +0.33 & 39.61 & 36.71
& -0.44 & 70.25 & 67.56
& -0.69 & 75.04 & 72.18
& -1.58 & 82.45 & 79.56
& -2.25 & 85.24 & 82.08 \\
& & ALDS-Simple3
& +0.09 & 49.09 & 51.10
& -0.21 & 57.83 & 57.04
& -0.94 & 74.48 & \textbf{74.79}
& -0.94 & 74.48 & 74.79
& -2.72 & 82.74 & 82.35 \\
& & ALDS-Simple5
& +0.02 & 39.42 & 38.65
& -0.30 & 64.39 & 64.05
& -0.95 & 70.03 & 71.61
& -1.07 & 74.48 & 74.79
& -2.51 & 82.74 & 82.35 \\
& & Messi3
& +0.01 & 40.31 & 40.80
& -0.38 & 63.99 & 65.53
& -0.91 & 70.08 & 71.84
& -1.21 & 75.63 & 75.23
& -2.70 & 78.57 & 80.38 \\
& & SVD-Error
& +0.00 & 49.36 & 48.27
& -0.19 & 57.52 & 56.72
& -0.76 & 64.45 & 63.88
& -1.76 & 70.25 & 68.97
& -2.86 & 75.00 & 74.31 \\
\hline
\end{tabular}


==> fig/imagenet_prune/imagenet_prune_table.tex <==
\begin{tabular}{|c|c|c||ccc|ccc|ccc|ccc|ccc|}
\hline
\multirow{9}{*}{\rotatebox{90}{ImageNet}}
& \multirow{2}{*}{Model}
& \multirow{2}{*}{\shortstack{Prune \\ Method}}
& \multicolumn{3}{c|}{$\delta=1.0\%$}
& \multicolumn{3}{c|}{$\delta=5.0\%$}
& \multicolumn{3}{c|}{$\delta=10.0\%$}
& \multicolumn{3}{c|}{$\delta=20.0\%$}
& \multicolumn{3}{c|}{$\delta=30.0\%$} \\
& &
& Top1/5 Acc. & CR-P & CR-F
& Top1/5 Acc. & CR-P & CR-F
& Top1/5 Acc. & CR-P & CR-F
& Top1/5 Acc. & CR-P & CR-F
& Top1/5 Acc. & CR-P & CR-F \\ \cline{2-18}
& \multirow{7}{*}{\shortstack{ResNet18 \\ \\ Top1: 69.62 \\ Top5: 89.08}}
& ALDS
& -0.65/-0.35 & \textbf{42.72} & \textbf{17.35}
& -4.42/-2.69 & \textbf{56.16} & \textbf{28.68}
& -4.42/-2.69 & \textbf{56.16} & \textbf{28.68}
& -12.64/-8.78 & \textbf{61.62} & \textbf{36.56}
& -22.54/-16.70 & \textbf{66.48} & \textbf{43.39} \\
& & PCA
&   &   &  
& -2.82/-1.18 & 2.00 & 3.00
& -5.95/-3.10 & 14.26 & 14.94
& -18.02/-11.80 & 34.43 & 34.74
& -26.09/-18.88 & 42.64 & \textbf{43.03} \\
& & SVD-Energy
&   &   &  
& -2.49/-1.55 & 1.99 & 2.51
& -2.49/-1.55 & 1.99 & 2.51
& -2.49/-1.55 & 1.99 & 2.51
& -25.34/-20.89 & 14.30 & 15.30 \\
& & SVD
&   &   &  
& -1.94/-1.20 & 2.00 & 2.16
& -8.28/-5.28 & 14.27 & 14.44
& -8.28/-5.28 & 14.27 & 14.44
& -23.11/-17.54 & 25.00 & 25.06 \\
& & L-Rank
&   &   &  
&   &   &  
&   &   &  
& -17.90/-13.57 & 2.00 & 9.31
& -17.90/-13.57 & 2.00 & 9.31 \\
& & FT
&   &   &  
& -1.55/-0.90 & 1.64 & 2.95
& -1.55/-0.90 & 1.64 & 2.95
& -1.55/-0.90 & 1.64 & 2.95
& -29.53/-23.34 & 14.21 & 14.89 \\
& & PFP
&   &   &  
& -3.21/-1.80 & 1.84 & 2.42
& -3.21/-1.80 & 1.84 & 2.42
& -3.21/-1.80 & 1.84 & 2.42
& -3.21/-1.80 & 1.84 & 2.42 \\
\hline
\end{tabular}


==> fig/voc_prune/voc_prune_table.tex <==
\begin{tabular}{|c|c|c||ccc|ccc|ccc|ccc|ccc|}
\hline
\multirow{9}{*}{\rotatebox{90}{VOCSegmentation2012}}
& \multirow{2}{*}{Model}
& \multirow{2}{*}{\shortstack{Prune \\ Method}}
& \multicolumn{3}{c|}{$\delta=1.0\%$}
& \multicolumn{3}{c|}{$\delta=5.0\%$}
& \multicolumn{3}{c|}{$\delta=10.0\%$}
& \multicolumn{3}{c|}{$\delta=20.0\%$}
& \multicolumn{3}{c|}{$\delta=30.0\%$} \\
& &
& IoU/Top1 Acc. & CR-P & CR-F
& IoU/Top1 Acc. & CR-P & CR-F
& IoU/Top1 Acc. & CR-P & CR-F
& IoU/Top1 Acc. & CR-P & CR-F
& IoU/Top1 Acc. & CR-P & CR-F \\ \cline{2-18}
& \multirow{7}{*}{\shortstack{DeeplabV3-ResNet50 \\ \\ IoU: 68.16 \\ Top1: 94.25}}
& ALDS
& -0.47/-0.19 & 27.39 & 27.30
& -4.79/-1.37 & 53.71 & 53.62
& -4.79/-1.37 & 53.71 & 53.62
& -4.79/-1.37 & 53.71 & 53.62
& -26.08/-7.10 & 60.15 & 60.00 \\
& & PCA
& -0.72/-0.35 & \textbf{60.10} & \textbf{60.25}
& -4.07/-1.31 & \textbf{70.42} & \textbf{70.74}
& -7.85/-2.18 & \textbf{74.53} & \textbf{74.92}
& -12.77/-3.31 & \textbf{78.07} & \textbf{78.53}
& -22.21/-5.79 & \textbf{81.11} & \textbf{81.61} \\
& & SVD-Energy
&   &   &  
&   &   &  
&   &   &  
& -11.33/-3.68 & 15.64 & 16.25
& -21.48/-6.86 & 27.40 & 28.05 \\
& & SVD
& -0.71/-0.18 & 15.54 & 15.42
& -0.71/-0.18 & 15.54 & 15.42
& -6.84/-1.68 & 27.31 & 27.18
& -10.59/-2.62 & 37.51 & 37.42
& -25.61/-6.90 & 46.25 & 46.19 \\
& & L-Rank
& -0.62/-0.20 & 27.42 & 27.34
& -2.48/-0.93 & 37.52 & 37.46
& -6.29/-1.67 & 46.22 & 46.27
& -19.75/-5.32 & 65.71 & 66.16
& -19.75/-5.32 & 65.71 & 66.16 \\
& & FT
& -0.29/-0.28 & 1.74 & 1.85
& -0.29/-0.28 & 1.74 & 1.85
& -0.29/-0.28 & 1.74 & 1.85
& -0.29/-0.28 & 1.74 & 1.85
& -23.51/-11.45 & 15.74 & 15.82 \\
& & PFP
& -0.08/-0.08 & 2.35 & 2.12
& -3.58/-0.92 & 15.84 & 15.01
& -3.58/-0.92 & 15.84 & 15.01
& -3.58/-0.92 & 15.84 & 15.01
& -22.62/-7.68 & 27.71 & 26.61 \\
\hline
\end{tabular}


==> sec/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}



\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See Section~\ref{sec:method_alds} and~\ref{sec:conclusion}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See supplementary material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{see supplementary material.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See supplementary material.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{We include an implementation for our method and many other competing methods.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}
